Proving Test Set Contamination in Black Box Language Models

Large language models are trained on vast amounts of internet data, prompting concerns and speculation that they have memorized public benchmarks. Going from speculation to proof of contamination is challenging, as the pretraining data used by proprietary models are often not publicly accessible. We show that it is possible to provide provable guarantees of test set contamination in language models without access to pretraining data or model weights. Our approach leverages the fact that when there is no data contamination, all orderings of an exchangeable benchmark should be equally likely. In contrast, the tendency for language models to memorize example order means that a contaminated language model will find certain canonical orderings to be much more likely than others. Our test flags potential contamination whenever the likelihood of a canonically ordered benchmark dataset is significantly higher than the likelihood after shuffling the examples. We demonstrate that our procedure is sensitive enough to reliably prove test set contamination in challenging situations, including models as small as 1.4 billion parameters, on small test sets of only 1000 examples, and datasets that appear only a few times in the pretraining corpus. Using our test, we audit five popular publicly accessible language models for test set contamination and find little evidence for pervasive contamination.

==> Makefile <==
TEXTIDOTE_VERSION := $(shell textidote --version 2>/dev/null)
IGNORE_RULES="sh:c:noin,lt:en:MORFOLOGIK_RULE_EN_US,lt:en:EN_UNPAIRED_BRACKETS,lt:en:CURRENCY,lt:en:PUNCTUATION_PARAGRAPH_END,sh:seclen"

main.pdf: clean
	latexmk -pdf main 2>&1 | awk 'BEGIN{IGNORECASE=1}/warning|!/,/^$$/;'

update:
	cd tex-common && git pull

clean:
	rm main.pdf *.aux *.bbl *.blg *.dvi *.fdb_latexmk *.fls *.log || true

linter:
	chktex -l .chktexrc -V  main.tex

spell:
	./.githooks/spelling.sh .

textidote.jar:
	wget "https://github.com/sylvainhalle/textidote/releases/download/v0.8.1/textidote.jar"

style: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output singleline main.tex

fullstyle: textidote.jar
	java -jar textidote.jar --check en --ignore ${IGNORE_RULES} --output plain main.tex

emacs:
	emacs --batch -l ~/.emacs --eval "(TeX-auto-generate \"tex-common/macros.sty\" \"auto\")"

makereview:
	git checkout -b reviewed && git push --set-upstream origin reviewed

